Streaming Factor Trajectory Learning for Temporal Tensor Decomposition

Practical tensor data is often along with time information. Most existing temporal decomposition approaches estimate a set of fixed factors for the objects in each tensor mode, and hence cannot capture the temporal evolution of the objects' representation. More important, we lack an effective approach to capture such evolution from streaming data, which is common in real-world applications. To address these issues, we propose Streaming Factor Trajectory Learning for temporal tensor decomposition. We use Gaussian processes (GPs) to model the trajectory of factors so as to flexibly estimate their temporal evolution. To address the computational challenges in handling streaming data, we convert the GPs into a state-space prior by constructing an equivalent stochastic differential equation (SDE). We develop an efficient online filtering algorithm to estimate a decoupled running posterior of the involved factor states upon receiving new data. The decoupled estimation enables us to conduct standard Rauch-Tung-Striebel smoothing to compute the full posterior of all the trajectories in parallel, without the need for revisiting any previous data. We have shown the advantage of SFTL in both synthetic tasks and real-world applications. The code is available at {https://github.com/xuangu-fang/Streaming-Factor-Trajectory-Learning}.

==> exp-zhe-backup.tex <==
%\vspace{-0.1in}
\vspace{-0.1in}
\section{Experiment}
\vspace{-.05 in}
\subsection{Ablation Study}
\vspace{-0.05in}
We first conducted an ablation study, for which we simulated a two-mode tensor, with two nodes per mode. Each node is represented by a time-varying factor, defined as follows.
\begin{align}
	&u^1_1(t) = -\sin^{3}(2\pi t), \; u^1_2(t) = \left(1-\sin^{3}(\frac{1}{2}\pi t)\right) \sin^{3}(3\pi t), \notag \\ 
	&u^2_1(t) = \sin(2\pi t), \; u^2_2(t) = -\cos^{3}(3\pi t) \sin(3\pi t)\sin(2\pi t). \notag 
\end{align}
Given these factors, a noisy entry value at an arbitrary time $t$ is generated via
\begin{align}
y_{(i, j)}(t) = u^1_i(t) u^2_j(t) + \epsilon, \;\; \epsilon \sim \N(\cdot | 0, 0.05). \label{eq:sample-entry}
\end{align}
We randomly sampled $500$ (irregular) timestamps from $[0, 1]$. For each specific timestamp $t$, we randomly picked two entries, and sampled their values according to \eqref{eq:sample-entry}. Overall, we sampled 1,000 observed tensor entry values. 

We implemented \ours with PyTorch~\citep{paszke2019pytorch}. We used $\nu = \frac{3}{2}$ and $a = \rho  = 0.3$ for the Mat\'ern kernel. We streamed the sampled entries according to their timestamps, and ran our streaming factor trajectory inference based on the CP form. The estimated trajectories  are shown in Fig. \ref{fig:simu-traj}.  As we can see, \ours recovers the ground-truth pretty accurately, showing that \ours has successfully captured the temporal evolution of the factor representation for every node. It is interesting to observe that when $t$ is around $0$, $0.5$ and $1$, the posterior standard deviation (the shaded region) increases significantly. This is reasonable: the ground-truth trajectories overlap at these time points, making it more difficult to differentiate/estimate their values at these time points. Accordingly, the uncertainty  of the estimation increases.

%\begin{figure}
\begin{table*}[]
	\centering
	\begin{small}
		\begin{tabular}{llcccc}
			\toprule
			& {RMSE}&  \textit{FitRecord} & \textit{ServerRoom} & \textit{BeijingAir-2} & \textit{BeijingAir-3}  \\ 
			\midrule
			\multirow{ 8}{*}{Static}&PTucker &    $ 0.656\pm0.147 $ & $ 0.458\pm0.039 $ & $ 0.401\pm0.01 $  & $ 0.535\pm0.062 $ \\
			&Tucker-ALS& $ 0.846\pm0.005 $ & $ 0.985\pm0.014 $ & $ 0.559\pm0.021 $ & $ 0.838\pm0.026 $ \\
			&CP-ALS  &       $ 0.882\pm0.017 $ & $ 0.994\pm0.015 $ & $ 0.801\pm0.082 $ & $ 0.875\pm0.028 $ \\
			&CT-CP       &               $ 0.664\pm0.007 $ & $ 0.384\pm0.009 $ & $ 0.64\pm0.007 $  & $ 0.815\pm0.018 $ \\
			&CT-GP          &            $ 0.604\pm0.004 $ & $ 0.223\pm0.035 $ & $ 0.759\pm0.02 $  & $ 0.892\pm0.026 $ \\
			&BCTT        &           $ 0.518\pm0.007 $ & $ 0.185\pm0.013 $ & $ 0.396\pm0.022 $ & $ 0.801\pm0.02 $  \\
			&NONFAT     &            $ 0.503\pm0.002 $ & $ \mathbf{0.117\pm0.006 }$ & $ 0.395\pm0.007 $ & $ 0.882\pm0.014 $ \\
			&THIS-ODE    &  $ 0.526\pm0.004 $         & $ 0.132\pm0.003 $ & $ 0.54\pm0.014 $         & $ 0.877\pm0.026 $ \\ 
			\hline
			\multirow{5}{*}{Stream}&POST        &            $ 0.696\pm0.019 $ & $ 0.64\pm0.028 $  & $ 0.516\pm0.028 $ & $ 0.658\pm0.103 $ \\
			&ADF-CP   &            $ 0.648\pm0.008 $ & $ 0.654\pm0.008 $ & $ 0.548\pm0.015 $ & $ 0.551\pm0.043 $ \\
			&BASS-Tucker        &            $ 0.976\pm0.024 $ & $ 1.000\pm0.016 $     & $ 1.049\pm0.037 $ & $ 0.991\pm0.039 $ \\
			&SFTL-CP     &  $ \mathbf{0.424\pm0.014} $ & $ 0.161\pm0.014 $ & $ \mathbf{0.248\pm0.012} $ & $ 0.473\pm0.013 $ \\
			&SFTL-Tucker &  $ 0.430\pm0.010 $   & $ 0.331\pm0.056 $ & $ 0.303\pm0.041 $ & $ \mathbf{0.439\pm0.019} $ \\ 
			\midrule
			& {MAE}    &           \\ 
			\midrule
			\multirow{ 8}{*}{Static}&PTucker &            $ 0.369\pm0.009 $ & $ 0.259\pm0.008 $ & $ 0.26\pm0.006 $  & $ 0.263\pm0.02 $  \\
			&Tucker-ALS &  $ 0.615\pm0.006 $ & $ 0.739\pm0.008 $ & $ 0.388\pm0.008 $ & $ 0.631\pm0.017 $ \\
			&CP-ALS  &            $ 0.642\pm0.012 $ & $ 0.746\pm0.009 $ & $ 0.586\pm0.056 $ & $ 0.655\pm0.018 $ \\
			&CT-CP       &            $ 0.46\pm0.004 $  & $ 0.269\pm0.003 $ & $ 0.489\pm0.006 $ & $ 0.626\pm0.01 $  \\
			&CT-GP          & $ 0.414\pm0.001 $ & $ 0.165\pm0.034 $ & $ 0.55\pm0.012 $  & $ 0.626\pm0.011 $ \\
			&BCTT        &            $ 0.355\pm0.005 $ & $ 0.141\pm0.011 $ & $ 0.254\pm0.007 $ & $ 0.578\pm0.009 $ \\
			&NONFAT     &            $ 0.341\pm0.001 $ & $ \mathbf{0.071\pm0.004} $ & $ 0.256\pm0.004 $ & $ 0.626\pm0.007 $ \\
			&THIS-ODE    & $ 0.363\pm0.004 $         & $ 0.083\pm0.002 $ & $ 0.345\pm0.004 $         & $ 0.605\pm0.013 $ \\
			\hline
			\multirow{5}{*}{Stream}&POST        &            $ 0.478\pm0.014 $ & $ 0.476\pm0.023 $ & $ 0.352\pm0.022 $ & $ 0.486\pm0.095 $ \\
			&ADF-CP              & $ 0.449\pm0.006 $ & $ 0.496\pm0.007 $ & $ 0.385\pm0.012 $ & $ 0.409\pm0.029 $ \\
			&BASS        &           $ 0.772\pm0.031 $ & $ 0.749\pm0.01 $  & $ 0.934\pm0.037 $ & $ 0.731\pm0.02 $  \\
			&SFTL-CP   &   $ \mathbf{0.242\pm0.006} $ & $ 0.108\pm0.008 $ & $\mathbf{ 0.15\pm0.003} $  & $ 0.318\pm0.008 $ \\
			&SFTL-Tucker &         $ 0.246\pm0.001 $ & $ 0.216\pm0.034 $ & $ 0.185\pm0.029 $ & $ \mathbf{0.278\pm0.011} $ \\ 
			\bottomrule
		\end{tabular}
	\end{small}
	%\vspace{-0.1in}
	\caption{\small Final prediction error \cmt{of the static and streaming decomposition methods,} with $R=5$. The results were averaged from five runs.}
	\label{table:Rank5res}
	%\vspace{-0.1in}
\end{table*}
\begin{wrapfigure}{r}{0.5\linewidth}
	\centering
	\setlength{\tabcolsep}{0pt}
	\begin{tabular}[c]{cc}
		\begin{subfigure}[b]{0.22\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/simu_U11.pdf}
			\caption{$u_1^1(t)$}
			\label{fig:simu-U11}
		\end{subfigure} &
		\begin{subfigure}[b]{0.22\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/simu_U12.pdf}
			\caption{$u_2^1(t)$}
			\label{fig:simu-U12}
		\end{subfigure} \\
		\begin{subfigure}[b]{0.22\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/simu_U21.pdf}
			\caption{$u_1^2(t)$}
			\label{fig:simu-U21}
		\end{subfigure} &
		\begin{subfigure}[b]{0.22\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/simu_U22.pdf}
			\caption{$u_2^2(t)$}
			\label{fig:simu-U22}
		\end{subfigure} \\
	\end{tabular}
	\vspace{-0.1in}
	\caption{\small The learned factor trajectories from the synthetic data. The shaded region indicates two posterior standard deviations. }\label{fig:simu-traj}
	\vspace{-0.2in}
\end{wrapfigure}
\begin{figure*}[!ht]
	\centering
	\setlength\tabcolsep{0pt}
	\begin{tabular}[c]{cccc}
		%\multicolumn{4}{c}{\includegraphics[width=0.718\textwidth]{./figs_new/legend2.pdf}}\\
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/flying_fitRecord_5.pdf}
			\caption{\textit{FitRecord} }
		\end{subfigure} 
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/flying_server_5.pdf}
			\caption{\textit{ServerRoom}}
		\end{subfigure} 
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/flying_beijing20k_5.pdf}
			\caption{\textit{BeijingAir-2} }
		\end{subfigure}
		&
		\begin{subfigure}[t]{0.24\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/flying_beijing15k_5.pdf}
			\caption{\textit{BeijingAir-3} }
		\end{subfigure}
	\end{tabular}	
	\vspace{-0.1in}
	\caption{\small Online prediction error with the number of processed entries ($R=5$).} 	
	\label{fig:running-performance-r5}
	\vspace{-0.2in}
\end{figure*}

\cmt{
\begin{table*}[]
	\centering
	\begin{small}
		\begin{tabular}{lcccc}
			\toprule
			RMSE&  \textit{FitRecord} & \textit{ServerRoom} & \textit{BeijingAir-2} & \textit{BeijingAir-3}  \\ 
			\midrule
			PTucker &    $ 0.656\pm0.147 $ & $ 0.458\pm0.039 $ & $ 0.401\pm0.01 $  & $ 0.535\pm0.062 $ \\
			Tucker-ALS& $ 0.846\pm0.005 $ & $ 0.985\pm0.014 $ & $ 0.559\pm0.021 $ & $ 0.838\pm0.026 $ \\
			CP-ALS  &       $ 0.882\pm0.017 $ & $ 0.994\pm0.015 $ & $ 0.801\pm0.082 $ & $ 0.875\pm0.028 $ \\
			CT-CP       &               $ 0.664\pm0.007 $ & $ 0.384\pm0.009 $ & $ 0.64\pm0.007 $  & $ 0.815\pm0.018 $ \\
			CT-GP          &            $ 0.604\pm0.004 $ & $ 0.223\pm0.035 $ & $ 0.759\pm0.02 $  & $ 0.892\pm0.026 $ \\
			BCTT        &           $ 0.518\pm0.007 $ & $ 0.185\pm0.013 $ & $ 0.396\pm0.022 $ & $ 0.801\pm0.02 $  \\
			NONFAT     &            $ 0.503\pm0.002 $ & $ \mathbf{0.117\pm0.006 }$ & $ 0.395\pm0.007 $ & $ 0.882\pm0.014 $ \\
			THIS-ODE    &  $ 0.526\pm0.004 $         & $ 0.132\pm0.003 $ & $ 0.54\pm0.014 $         & $ 0.877\pm0.026 $ \\ 
			\hline
			POST        &            $ 0.696\pm0.019 $ & $ 0.64\pm0.028 $  & $ 0.516\pm0.028 $ & $ 0.658\pm0.103 $ \\
			ADF-CP   &            $ 0.648\pm0.008 $ & $ 0.654\pm0.008 $ & $ 0.548\pm0.015 $ & $ 0.551\pm0.043 $ \\
			BASS-Tucker        &            $ 0.976\pm0.024 $ & $ 1.000\pm0.016 $     & $ 1.049\pm0.037 $ & $ 0.991\pm0.039 $ \\
			SFTL-CP     &  $ \mathbf{0.424\pm0.014} $ & $ 0.161\pm0.014 $ & $ \mathbf{0.248\pm0.012} $ & $ 0.473\pm0.013 $ \\
			SFTL-Tucker &  $ 0.430\pm0.010 $   & $ 0.331\pm0.056 $ & $ 0.303\pm0.041 $ & $ \mathbf{0.439\pm0.019} $ \\ 
			\midrule
			MAE    &           \\ 
			\midrule
			PTucker &            $ 0.369\pm0.009 $ & $ 0.259\pm0.008 $ & $ 0.26\pm0.006 $  & $ 0.263\pm0.02 $  \\
			Tucker-ALS &  $ 0.615\pm0.006 $ & $ 0.739\pm0.008 $ & $ 0.388\pm0.008 $ & $ 0.631\pm0.017 $ \\
			CP-ALS  &            $ 0.642\pm0.012 $ & $ 0.746\pm0.009 $ & $ 0.586\pm0.056 $ & $ 0.655\pm0.018 $ \\
			CT-CP       &            $ 0.46\pm0.004 $  & $ 0.269\pm0.003 $ & $ 0.489\pm0.006 $ & $ 0.626\pm0.01 $  \\
			CT-GP          & $ 0.414\pm0.001 $ & $ 0.165\pm0.034 $ & $ 0.55\pm0.012 $  & $ 0.626\pm0.011 $ \\
			BCTT        &            $ 0.355\pm0.005 $ & $ 0.141\pm0.011 $ & $ 0.254\pm0.007 $ & $ 0.578\pm0.009 $ \\
			NONFAT     &            $ 0.341\pm0.001 $ & $ \mathbf{0.071\pm0.004} $ & $ 0.256\pm0.004 $ & $ 0.626\pm0.007 $ \\
			THIS-ODE    & $ 0.363\pm0.004 $         & $ 0.083\pm0.002 $ & $ 0.345\pm0.004 $         & $ 0.605\pm0.013 $ \\
			\hline
			POST        &            $ 0.478\pm0.014 $ & $ 0.476\pm0.023 $ & $ 0.352\pm0.022 $ & $ 0.486\pm0.095 $ \\
			ADF-CP              & $ 0.449\pm0.006 $ & $ 0.496\pm0.007 $ & $ 0.385\pm0.012 $ & $ 0.409\pm0.029 $ \\
			BASS        &           $ 0.772\pm0.031 $ & $ 0.749\pm0.01 $  & $ 0.934\pm0.037 $ & $ 0.731\pm0.02 $  \\
			SFTL-CP   &   $ \mathbf{0.242\pm0.006} $ & $ 0.108\pm0.008 $ & $\mathbf{ 0.15\pm0.003} $  & $ 0.318\pm0.008 $ \\
			SFTL-Tucker &         $ 0.246\pm0.001 $ & $ 0.216\pm0.034 $ & $ 0.185\pm0.029 $ & $ \mathbf{0.278\pm0.011} $ \\ 
			\bottomrule
		\end{tabular}
	\end{small}
	%\vspace{-0.1in}
	\caption{\small Final prediction error with $R=5$. The results were averaged from five runs.}
	\label{table:Rank5res}
	%\vspace{-0.1in}
\end{table*}
}


%\vspace{-0.1in}
\subsection{Real-World Applications}
Next, we examined \ours in four real-world applications. (1) \textit{FitRecord} (\url{https://sites.google.com/eng.ucsd.edu/fitrec-project/home}), workout logs of EndoMondo users' health status in outdoor exercises. We extracted a three-mode tensor among 500 users, 20 sports types, and 50 altitudes. The entry values are heart rates. There are $50$K observed entry values along with the timestamps. (2) \textit{ServerRoom} (\url{https://zenodo.org/record/3610078#.Y8SYt3bMJGi}),   temperature logs of Poznan Supercomputing and Networking Center. We extracted a three-mode tensor between 3 air conditioning modes (24$^\circ$, 27$^\circ$ and 30$^\circ$), 3 power usage levels (50\%, 75\%, 100\%) and 34 locations. We collected 10K entry values and their timestamps. (3) \textit{BeijingAir-2} (\url{https://archive.ics.uci.edu/ml/datasets/Beijing+Multi-Site+Air-Quality+Data}), air pollution measurement in Beijing from year 2014 to 2017. We extracted a two-mode tensor (monitoring site, pollutant), of size $12 \times 6$, and collected  $20$K observed entry values (concentration) and their timestamps. (4) \textit{BeijingAir-3}, extracted from the same data source as \textit{BeijingAir-2}, a three-mode tensor among 12 monitoring sites, 12 wind speeds and 6 wind directions. The entry value is the PM2.5 concentration. There are $15$K observed entry values at different timestamps. 


% (2)(3)\textit{BeijingAir}(\url{https://archive.ics.uci.edu/ml/datasets/Beijing+Multi-Site+Air-Quality+Data}) the hourly concentration measurements of 6 pollutants, such as PM2.5, SO2, along with weather features at 12 monitoring sites across Beijing from 2014 to 2017. We process it into two datasets with different settings and features. First, we follow the easier way, extract \textit{BeijingAir-2-mode}, a two-mode (site-id, pollutants-type) tensor with $20$K observed entries along their timestamps. Then, we include the complex weather features involved with fewer observations and make a more challenging dataset \textit{BeijingAir-3-mode}, a three-mode (site-id, wind-direction, wind-speed) tensor with $15$K observed entries along the timestamps. Entries represent the measure of PM2.5 with six different wind directions and 12 wind-speed regions at 12 sites. 

\textbf{Competing Methods.}  We first compared with the following state-of-the-art streaming tensor decomposition methods based on the CP or Tucker model. (1) {POST} ~\citep{du2018probabilistic}, probabilistic streaming CP decomposition via mean-field streaming variational Bayes~\citep{broderick2013streaming} (2) {BASS-Tucker} ~\citep{fang2021bayesian} Bayesian streaming Tucker decomposition, which online estimates a sparse tensor-core via a spike-and-slab prior to enhance the interpretability. We also implemented (3) ADF-CP, streaming CP decomposition by combining  the assumed density filtering~\citep{boyen1998tractable} and conditional moment matching~\citep{wang2019conditional}.  %These methods online estimate a static factor representation for the objects appearing in the observed tenor entries, and they do not consider timestamps of the entries. To incorporate the time information for a fair comparison, we 

Next, we tested the state-of-the-art static decomposition algorithms, which have to go through the data many times. (4) P-Tucker~\citep{oh2018scalable}, an efficient Tucker decomposition algorithm that performs parallel row-wise updates. (5) CP-ALS and (6) Tucker-ALS~\citep{bader2008efficient},  CP/Tucker decomposition via alternating least square (ALS) updates. The methods  (1-6) are not specifically designed for temporal decomposition and cannot utilize the timestamps of the observed entries. In order to incorporate the time information for a fair comparison, we augment the tensor  with a time mode, and convert the ordered, unique timestamps into increasing time steps. 

We then compare with the most recent continuous-time temporal decomposition methods. Note that none of these methods can handle data streams. They have to iteratively access the data to update the model parameters and factor estimates. (7)  {CT-CP}~\citep{zhang2021dynamic}, continuous-time CP decomposition, which uses polynomial splines to model the CP coefficients $\blambda$ (see \eqref{eq:cp-lam} as a temporal function, (8) {CT-GP}, continuous-time GP decomposition, which extends~\citep{zhe2016dintucker} to use GPs to learn the tensor entry value as a function of the latent factors and time $y_\bell(t) = g(\u^1_{\ell_1}, \ldots, \u^K_{\ell_K}, t) \sim \gp(0,\kappa(\cdot, \cdot))$, (9) {BCTT} ~\citep{fang2022bayesian}, Bayesian continuous-time Tucker decomposition, which estimates the tensor-core as a time-varying function, (10) {THIS-ODE}~\citep{li2022decomposing}, which uses a neural ODE~\citep{chen2018neural} to model the entry  value as a function of the latent factors and time, $\frac{\d y_\bell(t)}{\d t} = \text{NN}(\u^1_{\ell_1}, \ldots, \u^K_{\ell_K}, t)$ where NN is short for neural networks. (11)  {NONFAT}~\citep{wang2022nonparametric}, nonparametric factor trajectory learning, the only existing work that also estimates factor trajectories for temporal tensor decomposition. It uses a bi-level GP to estimate the trajectories in the frequency domain and applies inverse Fourier transform to return to the time domain. 


%Group \textbf{c} includes some state-of-art temporal tensor models, which can handle the continuous timestamps. (c1) \textit{CT-CP}.~\citep{zhang2021dynamic}, continuous-time CP decomposition, which uses polynomial splines to estimates $\blambda$ in \eqref{eq:cp} as a trend function. (c2) \textit{CT-GP} continuous-time GP decomposition, which extends~\citep{zhe2016dintucker} to use GPs to learn tensor element as a function of the latent factors and time $y_\bi(t) = g(\u^1_{i_1}, \ldots, \u^K_{i_K}, t) \sim \gp(0,\kappa(\cdot, \cdot))$. (c3) \textit{BCTT} ~\citep{fang2022bayesian} Bayesian continuous-time Tucker decomposition, modeling the tucker cores as the time-varying functions (b4) \textit{THIS-ODE}. (c4) \textit{THIS-ODE}.~\citep{li2022decomposing} (c5) \textit{NON-FAT}.~\citep{wang2022nonparametric}


%We want to verify \ours by asking three questions: \textbf{1: Dose the proposed streaming inference work well?}, \textbf{2: Is the SDE-GP-based trajectory learning an appropriate method to model continuous dynamics compared to others?}, and \textbf{3: Is that really helpful to handle the temporal info with a continuous form?} Correspondingly, we pick three different groups of state-of-the-art baselines. The group \textbf{a} includes three streaming probabilistic tensor learning algorithms, which can handle the streaming data and sequentially make predictions. (a1) \textit{POST} ~\citep{du2018probabilistic} Probabilistic Streaming CP Decomposition adopting streaming variational Bayes
%(SVB) approach. (a2) \textit{ADF-CP}, the CP decomposition model updating with assumed-density-filtering(ADF)~\citep{ghosh2016assumed} framework, which is also known as Bayesian Online Learning (a3) \textit{BASS} ~\citep{fang2021bayesian} Bayesian Streaming Sparse Tucker decomposition, which is a Bayesian Tucker model with sparse core and sequentially also updates with (ADF).  We expand the original tensor with an extra discrete-time mode for these streaming methods and feed in with the time-id order.


%Group \textbf{b}, we put some popular classic tensor decomposition models that discrete the timestamps and make it an extra mode. (b1) \textit{DDT-PTucker}~\citep{oh2018scalable} a scalable Tucker decomposition algorithm that performs parallel row-wise updates.(b2) \textit{DDT-Tucker-ALS} (b3) \textit{DDT-CP-ALS}. Efficient Tucker/CP decomposition algorithm using alternative least square(ALS) update.~\citep{bader2008efficient}

%Group \textbf{c} includes some state-of-art temporal tensor models, which can handle the continuous timestamps. (c1) \textit{CT-CP}.~\citep{zhang2021dynamic}, continuous-time CP decomposition, which uses polynomial splines to estimates $\blambda$ in \eqref{eq:cp} as a trend function. (c2) \textit{CT-GP} continuous-time GP decomposition, which extends~\citep{zhe2016dintucker} to use GPs to learn tensor element as a function of the latent factors and time $y_\bi(t) = g(\u^1_{i_1}, \ldots, \u^K_{i_K}, t) \sim \gp(0,\kappa(\cdot, \cdot))$. (c3) \textit{BCTT} ~\citep{fang2022bayesian} Bayesian continuous-time Tucker decomposition, modeling the tucker cores as the time-varying functions (b4) \textit{THIS-ODE}. (c4) \textit{THIS-ODE}.~\citep{li2022decomposing} (c5) \textit{NON-FAT}.~\citep{wang2022nonparametric}
 

%{\bf Settings.}
For all the competing methods, we used the publicly released  implementations of the original authors. The hyper-parameter setting and turning follows the original papers.  For \ours, we chose $\nu$ from $\{\frac{1}{2}, \frac{3}{2}\}$,  $a$ from [0.5, 1] and $\rho$ from [0.1, 0.5]. For our online filtering, the maximum number of CEP iterations was set to $50$ and the tolerance level to $10^{-4}$.  For numerical stability, we re-scaled the timestamps to $[0, 1]$. We examined the number of factors (or factor trajectories) $R \in \{2, 3, 5, 7\}$. 

%We used the official open-source implementations of most baselines, implemented \ours and (a2) by PyTorch. For GP-based models, we used SE kernel and sparse variational GP  inference as in~\citep{zhe2016distributed} for scalable model estimation, and set pseudo inputs was $100$. For CT-CP, we used $100$ knots for the polynomial splines. To ensure numerical stability, we re-scaled all the timestamps to $[0, 1]$. For \ours, we finetuning the models with Mat\'ern kernels $\nu = \{1/2, 3/2\}$ along the kernel parameters for optimal performance for different datasets. We examined all the methods with the number of factors $R \in \{2, 3, 5, 7\}$. Following ~\citep{xu2012infinite,kang2012gigatensor,zhe2016distributed}, we randomly sampled $80\%$ observed entry values and their time points for training and then tested on the remaining entries. We repeated the experiments for five times, and then examined the average root mean-square-error (RMSE), average mean-absolute-error (MAE), and their standard deviations. 


%\subsection{Final Prediction Accuracy}
\noindent\textbf{Final Prediction Accuracy.} We first examined the final prediction accuracy with our learned factor trajectories. To this end, we followed ~\citep{xu2012infinite,kang2012gigatensor,zhe2016distributed}, and randomly sampled $80\%$ observed entry values and their timestamps for streaming inference and then tested the prediction error on the remaining entries. We also compared with the static decomposition methods, which need to repeatedly access the training entries. We repeated the experiment five times, and computed the average root mean-square-error (RMSE), average mean-absolute-error (MAE), and their standard deviations. We ran our method based on both the CP and Tucker forms, denoted by \ours-CP and \ours-Tucker, respectively. 
We report the results for $R=5$ in Table \ref{table:Rank5res}. Due to the space limit, we leave the other results in the Appendix (Table \ref{table:Rank2res}, \ref{table:Rank3res} and \ref{table:Rank7res}). As we can see, \ours outperforms all the streaming approaches by a large margin. \ours even obtains significantly better prediction accuracy than all the static decomposition approaches, except that on \textit{Server Room}, \ours is second to THIS-ODE and NONFAT. Note that \ours only went through the training entries for once. Although NONFAT  can also estimate the factor trajectories, it uses GPs to perform black-box nonlinear decomposition and hence loses  the interpretability. Note that NONFAT in most case also  outperforms the other static decomposition methods that only estimate time-invariant factors. The superior performance of \ours and NONFAT shows the importance of capturing the time evolution of factors. 

%\subsection{Online Predictive Performance}
\noindent \textbf{Online Predictive Performance.} Next, we evaluated the online predictive performance of \ours. Whenever a batch of entries at a new timestamp has been processed, we examined the prediction accuracy on the test set, with our current estimate of the factor trajectories.   We repeated the evaluation for five times, and examine how the average prediction error varies along with the number of processed entries. We show the results for $R=5$ in Fig. \ref{fig:running-performance-r5}, and the others in Appendix (Fig. \ref{fig:running-performance-r2}, \ref{fig:running-performance-r3} and \ref{fig:running-performance-r7}). It is clear that \ours in most cases outperforms the competing streaming decomposition algorithms by a large margin throughout the course of running. Note that the online behavior of BASS-Tucker was quite unstable and so we excluded it in the figures. 
%Although the other methods also exhibit decreasing prediction errors with more and more entries were processed, their running performance is constantly worse  than \ours. 
It confirms the advantage of our streaming trajectory learning approach ---  even in the streaming scenario, incrementally capturing the time-variation of the factors can perform better than updating fixed, static factors. 


 %It is clear that \ours performs better and converges faster than \textit{ADF-CP} and \textit{POST} on all tasks and settings. 

%We show the average prediction error \textit{vs.} the number of entries in Fig. XX
%\textbf{Prediction performance} Due to the space limit, we list the results for $R=2,3,5,7$ in Table \ref{table:Rank2res}Table\ref{table:Rank3res}Table\ref{table:Rank5res}Table\ref{table:Rank7res}, and the remaining in the appendix. As we can see, in all cases, our approach \ours outperforms the competing methods in the streaming group. It even beats all methods in Discrete-time and continuous-time groups on FitRecord and two BeijingAir datasets, where methods have to go through the training data multi-epochs. However, our streaming inference only sees each data point once. \textit{NON-FAT} gets better performance than \ours on \textit{Server Room}, but it applies more complex non-linear decomposition, as \ours only adopts multilinear CP and Tucker. We noticed \textit{BASS} almost failed on each task. It may cause by \textit{BASS} being designed for extremely large sparse tensors (observation ratio $< {10}^{-3}$), as our datasets do not belong to such cases.      

%\textbf{Dynamic performance for streaming data}
%We then examined the dynamic performance of \ours compared to methods in the streaming group, and the results are shown in Fig \ref{fig:running-performance-r2}Fig \ref{fig:running-performance-r3}Fig \ref{fig:running-performance-r5}Fig \ref{fig:running-performance-r7}. As \textit{BASS} almost failed on all tasks, we only show the results of \textit{ADF-CP}, \textit{POST}, and \ours. Following the streaming manner, we sequentially fed the observed entries to models with timestamp order and evaluated the prediction performance on the fly. It's clear that \ours performs better and converges faster than \textit{ADF-CP} and \textit{POST} on all tasks and settings. 
\vspace{-0.05in}
\subsection{Investigation of Learning Results }
%\begin{figure}
\begin{wrapfigure}{r}{0.5\linewidth}
	%	\vspace{-0.2in}
	\centering
	\setlength{\tabcolsep}{0pt}
	\begin{tabular}[c]{ccc}
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_1_node_3_r_1.pdf}
			\caption{$u_{1,1}^{1}(t)$}
			\label{fig:traj-U1-1}
		\end{subfigure} &
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_1_node_3_r_2.pdf}
			\caption{$u_{1,2}^{1}(t)$}
			\label{fig:traj-U1-2}
		\end{subfigure} &
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_1_node_3_r_3.pdf}
			\caption{$u_{1,3}^{1}(t)$}
			\label{fig:traj-U1-3}
		\end{subfigure} \\
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_2_node_1_r_1.pdf}
			\caption{$u_{2,1}^{2}(t)$}
			\label{fig:traj-U2-1}
		\end{subfigure} &
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_2_node_1_r_2.pdf}
			\caption{$u_{2,2}^{2}(t)$}
			\label{fig:traj-U2-2}
		\end{subfigure} &
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_2_node_1_r_3.pdf}
			\caption{$u_{2,3}^{2}(t)$}
			\label{fig:traj-U2-3}
		\end{subfigure} \\
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_3_node_3_r_1.pdf}
			\caption{$u_{3,1}^{3}(t)$}
			\label{fig:traj-U3-1}
		\end{subfigure} &
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_3_node_3_r_2.pdf}
			\caption{$u_{3,2}^{3}(t)$}
			\label{fig:traj-U3-2}
		\end{subfigure} &
		\begin{subfigure}[b]{0.16\textwidth}
			\centering
			\includegraphics[width=\linewidth]{./figs/traj/mode_3_node_3_r_3.pdf}
			\caption{$u_{3,3}^{3}(t)$}
			\label{fig:traj-U3-3}
		\end{subfigure} 
	\end{tabular}
	\vspace{-0.1in}
	\caption{\small The learned factor trajectories of object 1, 2, 3 in mode 1, 2, 3, respectively, from  the \textit{ServerRoom} dataset. The shaded region shows one standard deviation and the dashed line indicates the biggest timestamp in the data.}
	\vspace{-0.1in}
	\label{fig:traj}
	%\vspace{0.05in}
\end{wrapfigure}
Finally, we investigated our learned factor trajectories. We set $R = 3$ and ran \ours-CP on \textit{ServerRoom}. In Fig. \ref{fig:traj}, we visualize the trajectory for the 1st air conditioning mode, the 2rd power usage level,  and the 3rd location. The shaded region indicates the standard deviation, and the red dashed line the biggest timestamp in the data. First, we can see that the posterior variance of all the trajectories grow quickly  when moving to the right of the red line. This is reasonable because it is getting far away from the training region. Second, for each object, the first and second trajectories (1st and 2nd column in Fig. \ref{fig:traj}) exhibit quite different time-varying patterns, \eg the local periodicity in $u^1_{1, 2}(t)$ and $u^2_{2,2}(t)$, the gradual decreasing and increasing trends in $u^3_{3,1}(t)$ and $u^3_{3,2}(t)$, respectively, which imply different inner properties of the object. Third, it is particularly interesting that the third trajectory for all the objects appear to be close to zero, with relatively large posterior variance all the time. This might imply that two factor trajectories have been sufficient to represent each object.  Requesting for a third trajectory is redundant.  More important, our model is able to detect such redundancy and gives a zero-valued trajectory. 
%in \ref{fig:traj}. The shaded region is the standard It confirms the advantage of our streaming trajectory inference approach, and also shows that even in the streaming scenario, incrementally capturing the time-variation of the factors can perform better than updating fixed, static factors. , and the red dashed line represents the last timestamp when that factor gets involved in the training set.
%There are several exciting explorations. 1) Among all the three factors, the trajectories of rank-$1$ and rank-$2$ Fig \ref{fig:traj-U1-1}Fig\ref{fig:traj-U1-2}Fig\ref{fig:traj-U2-1}Fig\ref{fig:traj-U2-2}Fig\ref{fig:traj-U3-1}Fig\ref{fig:traj-U1-2}  all present the trend and periodic properties, but rank-$3$ trajectories Fig\ref{fig:traj-U1-3}Fig\ref{fig:traj-U2-3}Fig\ref{fig:traj-U3-3} seems to be time-invariant and close to zero. It indicates that rank-$3$ trajector is redundant, and the optimal rank of this dataset may be $r=2$. 2) The uncertainty level (shaded region) boosts at the right side of the red line, where there are no observations in training. It's consistent with the fact that the model is more uncertain about the extrapolation, and may help the model interpretability for down-streaming tasks. 

==> method-backup.tex <==
%background: CP/Tucker/GP decompostion

%method: model --> spectral analysis to derive state-space prior --> inference algorithm
\vspace{-0.1in}
\section{Preliminaries}\label{sect:bk}
\vspace{-0.05in}
\textbf{Tensor Decomposition.} We denote an $M$-mode tensor by $\Ycal \in \mathbb{R}^{d_1 \times \cdots \times d_M}$, where each mode $m$ has $d_m$ dimensions, corresponding to $d_m$ objects. Each tensor entry is indexed by a tuple $\bell = \left(\ell_1, \ldots, \ell_M\right)$, and the value is denoted by $y_\bell$. For decomposition, we introduce a set of latent factors $\u^m_j \in \mathbb{R}^{R_m}$ to represent each object $j$ in mode $m$ ($1 \le m \le M$). One most popular tensor decomposition model is the CANDECOMP/PARAFAC (CP) decomposition~\citep{Harshman70parafac}, which sets $R_1 = \ldots = R_M = R$, and uses the following element-wise form, $y_{\bell} \approx \1^\top (\u^1_{\ell_1} \circ \ldots \circ \u^M_{\ell_M})= \sum\nolimits_{r=1}^{R}  \prod\nolimits_{m=1}^{M} u_{\ell_{m} r}^{m}$,
%\begin{align}
%	y_{\bell} \approx \blambda^\top (\u^1_{\ell_1} \circ \ldots \circ \u^M_{\ell_M})= \sum\nolimits_{r=1}^{R} \lambda_{r} \prod\nolimits_{m=1}^{M} u_{\ell_{m} r}^{m} \label{eq:cp-lam}
%\end{align}
where $\circ$ is the element-wise product. 
Another commonly used model is Tucker decomposition~\citep{Tucker66}, $y_\bell \approx \vec(\Wcal )^{\top}\left(\u_{\ell_{1}}^{1} \otimes \ldots \otimes \u_{\ell_{M}}^{M}\right) =\sum\nolimits_{r_{1}=1}^{R_{1}} \ldots \sum\nolimits_{r_{M}=1}^{R_{M}}\left[w_{\br} \cdot \prod\nolimits_{m=1}^{M} u_{\ell_{m}, r_{m}}^{m}\right]$, 
%\begin{align}
%	&y_\bell \approx \vec(\Wcal )^{\top}\left(\u_{\ell_{1}}^{1} \otimes \ldots \otimes \u_{\ell_{M}}^{M}\right) =\sum\nolimits_{r_{1}=1}^{R_{1}} \ldots \sum\nolimits_{r_{M}=1}^{R_{M}}\left[w_{\br} \cdot \prod\nolimits_{m=1}^{M} u_{\ell_{m}, r_{j}}^{m}\right] \label{eq:tucker} 
%\end{align}
where $\Wcal \in \mathbb{R}^{R_1 \times \cdots \times R_M} $ is the Tucker-core parameter, $\vec(\cdot)$ is the vectorization, $\otimes$ is the Kronecker product,  and $\r = (r_1, \ldots, r_M)$. %CP and Tucker decomposition models are simple, elegant, and provide good interpretability. %They estimate the interactions between the factors of different objects,  consider their additive effect  on the entry values, and hence can provide good interpretability. 


\textbf{Gaussian Process (GP)s} are  nonparametric function priors. For a function $f(\x)$, if we place a GP prior, $f \sim \gp(0, \kappa(\x, \x'))$, it means $f(\cdot)$ is sampled as a realization of the GP with covariance function $\kappa$, which is often chosen as a kernel function. The GP prior only models the correlation between the function values, namely, $\text{cov}\left(f(\x), f(\x')\right) = \kappa(\x, \x')$, and does not assume any parametric form of the function. Hence, GPs are flexible enough to estimate various complex functions from data, \eg from multilinear to highly nonlinear. The finite projection of the GP is a Gaussian distribution. That is, given an arbitrary collection of inputs $\{\x_1, \ldots, \x_N\}$, the corresponding function values $\f = [f(\x_1), \ldots, f(\x_N)]^\top$ follow a multi-variate Gaussian prior distribution, $p(\f) = \N(\f|\0, \K)$ where $\K$ is the covariance matrix and each $[\K]_{mn} = \kappa(\x_m, \x_n)$. 



%\vspace{-0.05in}
%\subsection{Tensor Decomposition}
%\vspace{-0.05in}
\cmt{
\noindent\textbf{Tensor Decomposition.} Consider a $K$-mode tensor $\mathcal{Y} \in \mathbb{R}^{d_{1} \times \cdots \times d_{K}}$, where $d_k$ is the number of nodes in mode $k$.  We use a $K$-elements tuple $\mathbf{i}=\left(i_{1}, \ldots, i_{K}\right)$ to index each entry of the tensor, and denote the entry value by $y_{\mathbf{i}}$. To factorize $\Ycal$ into a concise structure, we introduce a set of latent factors for the tensor nodes, $\Ucal = \{\U^{1}, \ldots,  \U^{K}\}$, where each $\U^k = [ \u^k_1, \ldots, \u^k_{d_k}]^\top$ is a factor matrix, in which each row consists of the factors for a node $j$ in mode $k$, namely $\u_j^k$ ($1\le j \le d_k$). Given the factorization form, we estimate the optimal factors $\Ucal$ to reconstruct the tensor $\Ycal$, by minimizing a loss on the observed entries. 
The (arguably) most popular tensor factorization model is CANDECOMP/PARAFAC (CP)~\citep{Harshman70parafac}, whose entry-wise form is given by
\begin{align}
	y_{\mathrm{i}} \approx \blambda^\top (\u^1_{i_1} \circ \ldots \circ \u^K_{i_K})= \sum\nolimits_{r=1}^{R} \lambda_{r} \prod\nolimits_{k=1}^{K} u_{i_{k}, r}^{k}, \label{eq:cp}
\end{align}
where $\circ$ is the Hadamard (element-wise) product, $\blambda = (\lambda_1, \ldots, \lambda_R)^\top$ and each $\u^k_{i_k} = (u^k_{i_k,1}, \ldots, u^k_{i_k,R})^\top$. 
While simple and convenient, CP only accounts for the interaction between every $r$-th factor in different modes, \ie $\prod_{k=1}^{K} u_{i_{k}, r}^{k}$ (weighted by $\lambda_r$ accordingly), and overlook all the other possible interactions.  

Tucker decomposition~\citep{Tucker66} is more interpretable and expressive than CP in that it considers all the possible interactions between the factors across the tensor modes. Specifically, Tucker decomposition assumes $ \mathcal{Y} \approx \mathcal{W} \times_{1} \mathbf{U}^{1} \times_{2} \ldots \times_{K} \mathbf{U}^{K}$ where $\Wcal \in \mathbb{R}^{R_1 \times \ldots \times R_K}$ is parametric tensor-core and $ \times_k$ is mode $k$ tensor-matrix product~\citep{kolda2006multilinear}. The entry-wise form is therefore given by
\begin{align}
	y_\bi &\approx \vec(\Wcal )^{\top}\left(\u_{i_{1}}^{1} \otimes \ldots \otimes \u_{i_{K}}^{K}\right) \notag \\
	&=\sum_{r_{1}=1}^{R_{1}} \ldots \sum_{r_{K}=1}^{R_{K}}\left[w_{(r_{1}, \ldots, r_{K})} \cdot \prod_{k=1}^{K} u_{i_{k}, r_{k}}^{k}\right] \label{eq:tucker} 
\end{align}
where $\vec(\cdot)$ is the vectorization and $\otimes$ is the Kronecker product. As we can see from \eqref{eq:tucker}, every interaction between the factors across the $K$ modes are accounted for, $\{\prod_{k=1}^{K} u_{i_{k}, r_{k}}^{k}|1\le r_1 \le R_1, \ldots, 1 \le r_K \le R_K\}$.\cmt{, which are in total $R_1 \times \ldots \times R_K$ interactions.} Each interaction is weighted by an element of the tensor-core. It is easy to see that CP is a special case of Tucker decomposition when we set all $R_k = R$ and $\Wcal$ to be diagonal. 
}
%\vspace{-0.1in}
%\subsection{Gaussian Process}
%\vspace{-0.05in}

%\textbf{Gaussian Processes (GPs)} are powerful Bayesian function estimators. Due to the nonparametric  nature, GPs can automatically grasp the complexity of the target function underlying  the data (\eg from linear to highly linear), not restricted to any parametric form.  Specifically, suppose given $N$ training examples, $\X =  \left[\x_{1}, \ldots, \mathbf{x}_{N}\right]^{\top}$ and $\mathbf{y}=\left[y_{1}, \ldots, y_{N}\right]^{\top}$, we want to learn a function $f: \mathbb{R}^d \rightarrow \mathbb{R}$. We place a GP prior over the target function, and then any finite set of the function values follow a multivariate Gaussian distribution. Consider $\f = [f(\x_1), \ldots, f(\x_N)]$ and we have $p(\f) = \N(\f|\m, \K)$,



%way up to consder the modeo joint probability --> inference hurdle --> state space prior --> new probability
\vspace{-0.1in}
\section{Bayesian Temporal Tensor Decomposition with Factor Trajectories}
\vspace{-0.05in}
In real-world applications, tensor data is often associated with time information, namely, the timestamps at which the objects of different modes interact to generate the entry values. %To incorporate this information in the decomposition, most methods bin the timestamps into a sequence of time steps and augment the tensor with a time mode. The recent a few methods integrate the continuous time points into the decomposition model [XX]. In spite of their success, all these method  still estimate a set of fixed factors for the objects in each  mode. However, since the inner properties of an object often vary with time, \eg product popularity, health status and income, learning a fixed factor representation can miss those important evolution patterns. To address this limitation, we propose a Bayesian temporal decomposition model with  factor trajectories. Specifically, to 
To capture the potential evolution of the objects' inner properties, we propose a Bayesian temporal tensor decomposition model that can estimate a trajectory of the factor representation. Specifically, for each object $j$ in mode $m$, we model the factors as a function of time, $\u^m_j : [0, \infty] \rightarrow \mathbb{R}^R$. To flexibly capture a variety of temporal evolution, we assign a GP prior over each element of $\u^m_j(t) = [u^m_{j1}(t), \ldots, u^m_{jR}(t)]^\top$,  and $u^m_{jr}(t) \sim \gp(0, \kappa(t, t'))$ ($1 \le r \le R$). 
%\begin{align}
	%u^m_{jr}(t) \sim \gp(0, \kappa(t, t')) \label{eq:gp-u}
%\end{align}
%where $1 \le r \le R$. 
Given the factor trajectories, we then use the CP or Tucker form to sample the entry values at different time points. For the CP form, we have  
\begin{align}
	&p(y_\bell(t)|\Ucal(t)) = \N(y_\bell(t) | \1^\top (\u^1_{\ell_1}(t) \circ \ldots \circ \u^K_{\ell_M}(t)), \tau^{-1}), \label{eq:cp-ll}
\end{align}
where $\Ucal(t) = \{\u^m_{j}(t)\}$ includes all the factor trajectories, and 
$\tau$ is the inverse noise variance, for which we assign a Gamma prior, $p(\tau) = \text{Gam}(\tau|\alpha_0, \alpha_1)$. For the Tucker form, we have $p(y_\bell(t)|\Ucal(t), \Wcal) = \N(y_\bell(t) | \vec(\Wcal)^\top (\u^1_{\ell_1}(t) \kron \ldots \kron \u^K_{\ell_M}(t)), \tau^{-1})$
%\begin{align}
%	&p(y_\bell(t)|\Ucal(t), \Wcal) \label{eq:tucker-ll}  \\
%	&= \N(y_\bell(t) | \vec(\Wcal)^\top (\u^1_{\ell_1}(t) \kron \ldots \kron \u^K_{\ell_M}(t)), \tau^{-1}), \notag
%\end{align}
where we place a standard normal prior over the tensor-core, $p(\vec(\Wcal)) = \N(\vec(\Wcal)|\0, \I)$.  In this work, we focus on continuous observations. It is straightforward to extend our method for  other types of observations. 

Suppose we have a collection of observed entry values and timestamps, $\Dcal = \{(\bell_1, y_1, t_1), \ldots, (\bell_N, y_N, t_N)\}$ where $t_1 \le \cdots \le t_N$.  We denote the sequence of timestamps when a particular object $j$ of mode $m$ participated in the observed entries by $s^m_{j,1} < \ldots < s^m_{j,c^m_j}$, where $c^m_j$ is the participation count of the object. Note that it is a sub-sequence of $\{t_n\}$. From the GP prior, the values of each $u^m_{jr}(t)$ at these timestamps follow a multi-variate Gaussian distribution, $p(\u^m_{jr}) = \N(\u^m_{jr}|\0, \K^m_{j})$ where $\u^m_{jr} = [u^m_{jr}(s^m_{j,1}), \ldots, u^m_{jr}(s^m_{j,c^m_j}) ]^\top$ and $\K^m_j$ is the kernel matrix computed at these timestamps. The joint probability of our model with the CP form is  
\begin{align}
	&p(\{\u^m_{jr}\},\tau, \y) = \prod\nolimits_{m=1}^M \prod\nolimits_{j=1}^{d_m} \prod\nolimits_{r=1}^R \N(\u^m_{jr}|\0, \K^m_j)  \text{Gam}(\tau|\alpha_0, \alpha_1)\notag \\
	&  \cdot \prod\nolimits_{n=1}^N \N(y_n | \1^\top (\u^1_{\ell_{n1}}(t_n) \circ \ldots \circ \u^M_{\ell_{nM}}(t_n)), \tau^{-1}). \label{eq:joint-1} \raisetag{0.2in}
\end{align}
The joint probability with the Tucker form is the same  except that we use the Tucker likelihood instead and multiply with the prior of  tensor-core $p(\Wcal)$.

While this formulation is straightforward, it can introduce computational challenges. There are many multi-variate Gaussian distributions in the joint distribution \eqref{eq:joint-1}, \ie $\{\N(\u^m_{jr}|\0, \K^m_j)\}$. The time and space complexity to compute each $\N(\u^m_{jr}|\0, \K^m_j)$ is $\Ocal\left(\left(c^m_j\right)^3\right)$ and $\Ocal\left(\left(c^m_j\right)^2\right)$, respectively. With the increase of $N$, the appearance count $c^m_j$ for many objects can grow as well, making the computation cost very expensive or even infeasible. The issue is particularly severe when we handle streaming data --- the number of timestamps grows rapidly with new data keeps coming in, so does the size of each covariance matrix. 

\subsection{Equivalent Modeling with State-Space Priors}
To sidestep expensive kernel matrix computation and ease the inference with streaming data, we follow~\citep{hartikainen2010kalman} to convert the GP prior into an SDE via spectral analysis. Specifically, we consider the popular Mat\'ern kernel family, 
\begin{align}
	\kappa_\nu\left(t, t'\right)&=a \frac{\left(\frac{\sqrt{2 \nu}}{\rho} \Delta \right)^{\nu}}{\Gamma(\nu) 2^{\nu-1}}
	K_{\nu}\left(\frac{\sqrt{2 \nu}}{\rho} \Delta\right) \label{Matern_kernel}
\end{align}
where $\Delta = |t - t'|$, $\Gamma(\cdot)$ is the Gamma function, $a>0$ and $\rho>0$ are the amplitude and length-scale parameters, respectively, $K_{\nu}$ is the modified Bessel function of the second kind, $\nu>0$ controls the smoothness.\cmt{ It means that if $f(t) \sim \gp(0, \kappa_\nu(t, t'))$, $f(t)$ is $\lceil \nu \rceil-1$ times differentiable in the mean-square sense []. }
Since $\kappa_\nu$ is a stationary kernel, \ie $\kappa_\nu(t, t') = \kappa_\nu(t - t')$, according to the  Wiener–Khinchin theorem~\citep{chatfield2003analysis}, if $f(t) \sim \gp(0, \kappa_\nu(t, t'))$, the energy spectrum density of $f(t)$ can be obtained by the Fourier transform of $\kappa_\nu(\Delta)$, 
\begin{align}
	S(\omega ) = a \frac{2\sqrt{\pi}\Gamma(\frac{1}{2} + \nu)}{\Gamma(\nu)} \alpha^{2\nu}\left(\alpha^2 + \omega^2\right)^{-\left(\nu + \frac{1}{2}\right)}
\end{align}
where $\omega$ is the frequency, and $\alpha = \frac{\sqrt{2\nu}}{\rho}$. We consider the commonly used choice  $\nu = p + \frac{1}{2}$ where $p \in \{0, 1, 2, \ldots\}$. Then we can observe that 
\begin{align}
	S(\omega) = \frac{\sigma^2}{(\alpha^2 + \omega^2)^{p+1}} = \frac{\sigma^2}{(\alpha + i \omega)^{p+1}(\alpha - i \omega)^{p+1}} \label{eq:spec-density}
\end{align}
where $\sigma^2 = a\frac{ 2\sqrt{\pi}\Gamma(p+1)}{\Gamma(p+\frac{1}{2})} \alpha^{2p + 1}$, and $i$ indicates an imaginary number. We expand the polynomial 
\begin{align}
	(\alpha + i \omega)^{p+1} = \sum\nolimits_{k=0}^p c_k (i\omega)^k + (i\omega)^{p+1} \label{eq:poly}
\end{align}
where $\{c_k|0 \le k \le p\}$ are the coefficients.  From \eqref{eq:spec-density} and \eqref{eq:poly}, we can construct an equivalent system to generate the signal $f(t)$. That is,  in the frequency domain, the system output's Fourier transform   $\widehat{f}(\omega)$ is given by 
\begin{align}
	\sum\nolimits_{k=1}^p c_k (i\omega)^k \widehat{f}(\omega) + (i\omega)^{p+1} \widehat{f}(\omega) = \widehat{\beta}(\omega) \label{eq:fourier}
\end{align}
where $\widehat{\beta}$ is the Fourier transform of a white noise process $\beta(t)$ with spectral density (or diffusion) $\sigma^2$. The reason is that by construction, $\widehat{f}(\omega) = \frac{\widehat{\beta}(\omega)}{(\alpha + i \omega)^{p+1}}$, which gives exactly the same spectral density as in \eqref{eq:spec-density},  $S(\omega) = |\widehat{f}(\omega)|^2$.\cmt{ $= \widehat{f}(\omega)\widehat{f}^\dagger(\omega)$, where $\dagger$ is the complex conjugate.}  We then conduct inverse Fourier transform on both sides of \eqref{eq:fourier} to obtain the representation in the time domain, 
\begin{align}
	\sum\nolimits_{k=1}^p c_k \frac{\d^k f}{\d t^k} + \frac{\d^{p+1}f}{\d t^{p+1}} = \beta(t), \label{eq:sde}
\end{align}
which is an SDE. Note that $\beta(t)$ has the density $\sigma^2$. We can further construct a new state $\z = (f, f^{(1)}, \ldots, f^{(p)})^\top$ (where each $f^{(k)} \overset{\Delta}{=} \d^k f/\d t^k$) and convert \eqref{eq:sde} into a linear time-invariant (LTI) SDE, 
\begin{align}
	\frac{\d \z}{\d t} = \A \z + \boldeta \cdot \beta(t)
\end{align}
where 
\begin{align}
	\A =\left(\begin{array}{cccc}
		0 & 1 & & \\
		& \ddots  & \ddots & \\
		&   & 0 & 1 \\
		-c_0 & \ldots & -c_{p-1} & -c_{p}
	\end{array}\right), \quad \boldeta =\left(\begin{array}{c}
		0 \\
		\vdots\\
		0 \\
		1\\
	\end{array}\right). \notag 
\end{align}
For a concrete example, if we take $p=1$ (and so $\nu = \frac{3}{2}$), then $\A = [0, 1; -\alpha^2, -2 \alpha]$, $\boldeta = [0; 1]$, and $\sigma^2 = 4 a \alpha^3$. 

%general form of SDE
The LTI-SDE is particularly useful  in that its finite set of states follow a Gauss-Markov chain, namely the state-space prior.  Specifically, given arbitrary $t_1 < \ldots < t_L$, we have 
\begin{align}
	p(\z(t_1), \ldots, \z(t_L)) = p(\z(t_1)) \prod\nolimits_{k=1}^{L-1} p(\z(t_{k+1})| \z(t_{k})) \notag 
\end{align}
where $p(\z(t_1)) = \N(\z(t_1)|\0, \P_\infty)$, $p(\z(t_{k+1})| \z(t_{k})) = \N(\z(t_{k+1}) |\F_{k} \z(t_{k}), \Q_k)$, 
%\begin{align}
%	p(\z(t_1)) &= \N(\z(t_1)|\0, \P_\infty), \notag \\
%	p(\z(t_{k+1})| \z(t_{k})) &= \N(\z(t_{k+1}) |\F_{k} \z(t_{k}), \Q_k)
%\end{align}
$\P_\infty$ is the stationary covariance matrix computed by solving the matrix Riccati equation~\citep{lancaster1995algebraic}\cmt{ (\eg $\P_\infty = [a, 0; 0, a\alpha^2]$ when $n=1$)}, $\F_n = \exp(\Delta_k \cdot \A )$ where $\Delta_k = t_{k+1} - t_k$, and $\Q_k = \P_\infty - \A_k \P_\infty \A_k^\top$.  Therefore, we  do not  need the full covariance matrix as in the standard GP prior, and the computation is much more efficient. The chain structure is also convenient to handle streaming data as we will explain later. Note that for other type of kernel functions, such as the square exponential (SE) kernel, we can approximate the inverse spectral density $1/S(\omega)$ with a polynomial of $\omega^2$ with negative roots, and follow the same way to construct an LTI-SDE and state-space prior. 

We therefore convert the GP prior over each factor trajectory $u^m_{jr}(t)$ into an LTI-SDE. We denote the corresponding state by $\z^m_{j,r}(t)$. For example, if we choose $p=1$ ($\nu = \frac{3}{2}$), $\z^m_{j,r}(t) = [u^m_{jr}(t); \d u^m_{jr}(t)/\d t]$. 
 For each object $j$ in mode $m$, we concatenate all the trajectory states into one,  $\z^m_j = [\z^m_{j,1}; \ldots; \z^m_{j,R}]$. On the timestamps $s^m_{j,1} < \ldots < s^m_{j,c^m_j}$ when the object interacted with others to generated tensor entry values, we have a state-space prior 
\begin{align}
	p(\overline{\z}^m_{j,1}) = \N(\bar{\z}^m_{j,1} | \0, \overline{\P}_\infty), \;\;	p(\overline{\z}^m_{j,k+1} | \overline{\z}^m_{j,k}) = \N(\overline{\z}^m_{j,k+1}| \overline{\F}^m_{j,k}  \overline{\z}^m_{j,k}, \overline{\Q}^m_{j,k}) \label{eq:state-space}
\end{align}
where $\overline{\z}^m_{j,k} {=} \z^m_j(s^m_{j,k})$, 
$\overline{\P}_\infty = \diag(\P_\infty, \ldots, \P_\infty)$, $\overline{\F}^m_{j,k} = \diag\left(\F^m_{j,k}, \ldots, \F^m_{j,k}\right)$, $\F^m_{j,k} = e^{ (s^m_{j,k+1} - s^m_{j,k})\A}$,  $\overline{\Q}^m_{j,k} = \diag\left(\Q^m_{j,k}, \ldots, \Q^m_{j,k}\right)$, and $\Q^m_{j,k}  = \P_\infty - \F^m_{j,k} \P_\infty \left(\F^m_{j,k}\right)^\top$. 
\begin{figure*}[h]
	\centering
	\setlength\tabcolsep{0pt}
	\captionsetup[subfigure]{aboveskip=0pt,belowskip=0pt}
	\begin{tabular}[c]{c}
		\begin{subfigure}[t]{\textwidth}
			\centering
			\includegraphics[width=\textwidth]{./figs/traj/graphical.pdf}
			%\caption{}
		\end{subfigure} 
	\end{tabular}
	%	\vspace{-0.1in}
	\caption{\small  A graphical model representation of our factor trajectory learning, from which we can see $\{\Theta_{n+1}, \Bcal_{n+1}\}$ are independent to $\Dcal_{t_{n}}$ conditioned on $\Theta_{n}$ and the noise inverse variance $\tau$, namely, $\Theta_{n+1}, \Bcal_{n+1} \perp 
		\Dcal_{t_n} | \Theta_n, \tau$.}
	\label{fig:graphical_model}
\end{figure*}

 Given the data $\Dcal = \{(\bell_1, y_1, t_1), \ldots, (\bell_N, y_N, t_N)\}$, the joint probability of our model based on the CP form is now 
\begin{align}
	&p(\{\overline{\z}^m_{j,k}\}, \tau, \y)  =p(\tau) \prod\nolimits_{m=1}^M \prod\nolimits_{j=1}^{d_m} p(\overline{\z}^m_{j,1}) \prod\nolimits_{k=1}^{c^m_j - 1} 	p(\overline{\z}^m_{j,k+1} | \overline{\z}^m_{j,k}) \notag \\
	%\text{Gam}(\tau|a_0, b_0)\notag \\
	& \cdot  \prod\nolimits_{n=1}^N \N(y_n | \1^\top (\u^1_{\ell_{n1}}(t_n) \circ \ldots \circ \u^M_{\ell_{nM}}(t_n)), \tau^{-1}). \label{eq:new-prob} \raisetag{0.22in}
\end{align}
Note in the likelihood, each $\u^j_{{\ell_{nj}}}(t_n) (1 \le j \le M)$ is contained in a corresponding state vector $\barz^j_{{\ell_{nj}}, k} = \z^j_{\ell_{nj}}(t_n)$ where $s^j_{\ell_{nj}, k} = t_n$. The joint probability based on the Tucker form is similar, which we omit to save the space. 


%\textcolor{blue}{key obs: if we can incrementally compute p(xi|Di), which is Gaussian, then to compute the full posterior , we just need one pass of RTS smoothing.... If the likelihood is standard Gaussian, sequentially compute each ... can be efficiently and computed by KF, however, in our case ...... it is not. We therefore approximate ....  We use conditional moment matching to implement an EP inference, which efficiently give an ... .  Specifically, ...Finally, we apply the ... to leverage the formula as in .....}
\begin{algorithm}[H]
	\caption{Streaming Factor Trajectory Learning (\ours)}
	\begin{algorithmic}[1]
		\STATE {\bfseries Input:} kernel hyper-parameters $a$, $\rho$, $\nu=p+\frac{1}{2}$
		\STATE $n \leftarrow 0$ 
		\WHILE {Receiving a new batch of entreis $\Bcal_{n+1}$}
		\IF{$n = 0$}
		\STATE Set $a_n = a_0$, $b_n = b_0$, $\widehat{\bmu}^{m}_{j,c^m_{j,n+1}} = \0$, and $\widehat{\V}^{m}_{j,c^m_{j,n+1}} = \overline{\P}_\infty$ in \eqref{eq:running-2}
		\STATE Goto 9
		\ENDIF
		\STATE  Retrieve the involved preceding factor states $\Theta_{n} = \{\barz^m_{c^m_{j,n}} | j \in \Ical^m_{n+1}\}_m$ and their running posterior, $p(\Theta_{n}, \tau|\Dcal_{t_{n}})\approx \text{Gam}(\tau|a_{n}, b_{n}) \prod_{m=1}^M \prod_{j \in \Ical^m_{n+1}} \N(\barz^m_{j, c^m_{j, n}} | \bmu^m_{j, c^m_{j, n}}, \V^m_{j, c^m_{j, n}}) $.
		%\begin{align}
		%	&p(\Theta_{n}, \tau|\Dcal_{t_{n}})\approx \text{Gam}(\tau|a_{n}, b_{n}) \notag \\
		%	&\cdot \prod_{m=1}^M \prod_{j \in \Ical^m_{n+1}} \N(\barz^m_{j, c^m_{j, n}} | \bmu^m_{j, c^m_{j, n}}, \V^m_{j, c^m_{j, n}}) \notag 
		%\end{align}
		When $n=0$, $p(\Theta_n, \tau|\Dcal_{t_n})$ is the prior distribution. 
		\STATE  According to \eqref{eq:running-2} and \eqref{eq:ll-approx}, use conditional Expectation Propagation to obtain the running posterior of the current factor states, $p(\Theta_{n+1}, \tau|\Dcal_{t_{n+1}})\approx \text{Gam}(\tau|a_{n+1}, b_{n+1}) \prod_{m=1}^M \prod_{j \in \Ical^m_{n+1}} \N(\barz^m_{j, c^m_{j, n+1}} | \bmu^m_{j, c^m_{j, n+1}}, \V^m_{j, c^m_{j, n+1}})$.
		%\begin{align}
		%	&p(\Theta_{n+1}, \tau|\Dcal_{t_{n+1}})\approx \text{Gam}(\tau|a_{n+1}, b_{n+1}) \notag \\
		%	&\prod_{m=1}^M \prod_{j \in \Ical^m_{n+1}} \N(\barz^m_{j, c^m_{j, n+1}} | \bmu^m_{j, c^m_{j, n+1}}, \V^m_{j, c^m_{j, n+1}}) \notag 
		%\end{align}
		\IF {Needed}
		\STATE Run RTS smoothing on any factor  state chain $\{\barz^m_{j, k}|k=1, 2, \ldots\}$ of interest 
		\ENDIF
		\STATE $n \leftarrow n + 1$
		\ENDWHILE
		\STATE Run RTS smoothing for every factor state chain $\{\barz^m_{j,k}|k = 0, 1, 2\}$ where $1\le m \le M$ and $1 \le j \le d_m$
		\STATE {\bfseries Return:} $\{q(\barz^m_{j,k}|\Dcal)|k=1, 2, \ldots\}_{1 \le m \le M, 1 \le j \le d_m}$, $q(\tau|\Dcal)$, where $\Dcal$ is all the data received.
	\end{algorithmic}	\label{alg:alg}
\end{algorithm}
\vspace{-0.1in}
\section{Trajectory Inference from Streaming Data}
\vspace{-0.05in}
%problem definition
In this section, we develop an efficient, scalable algorithm for factor trajectory estimation from streaming data. In general, we assume that we receive a sequence of (small) batches of observed tensor entries, $\{\Bcal_1, \Bcal_2, \ldots\}$, generated at different timestamps, $\{t_1, t_2, \ldots\}$. Each batch $\Bcal_n$ is generated at timestamp $t_n$ and $t_n < t_{n+1}$. \cmt{Note that the same entry can be observed as different values at multiple timestamps.}  Denote by  $\Dcal_{t_n}$ all the data up to timestamp $t_n$, \ie $\Dcal_{t_n} = \Bcal_1 \cup \ldots \cup \Bcal_{n}$.  Upon receiving  $\Bcal_{n+1}$\cmt{ --- a batch of newly observed entries at $t_{n+1}$},  we intend to update our model without revisiting $\Dcal_{t_n}$ so that we can provide the trajectory posterior\cmt{given all the data up to given $\Dcal_{t_{n+1}}$}, $\{p(\u^m_j(t) | \Dcal_{t_{n+1}})| \forall t\ge 0, 1 \le m \le M, 1 \le j \le d_m\}$, where $\Dcal_{t_{n+1}} = \Dcal_{t_{n}} \cup \Bcal_{n+1}$. %Accordingly, we are  We are able to c compute the predictive distribution for an arbitrary entry value at an arbitrary time point $t$. 

%our observation, and RTS 
To this end, we first observe that the standard state-space model with a Gaussian likelihood has already provided a highly efficient streaming inference framework. Denote by $\x_n$ and $\y_n$ the state and observation at each step $n$, respectively. To handle streaming observations $\{ \y_1, \y_2, \ldots \}$, we only need to compute and track the running posterior $p(\x_n | \y_{1:n})$  upon receiving each $\y_n$, where $\y_{1:n} $ denotes the total data up to step $n$.  This is called Kalman filtering~\citep{sarkka2013bayesian}, which only depends on the running posterior at step $n-1$, \ie $p(\x_{n-1} | \y_{1:n-1})$, and is highly efficient. After all the data is processed (suppose it ends at step $N$),  we can use Rauch–Tung–Striebel (RTS) smoother~\citep{sarkka2013bayesian} to efficiently compute the full posterior of each state, $p(\x_n|\y_{1:N})$,  from backward, which does not need to re-access any previous observation (see Sec. \ref{sect:rts} in Appendix).
\cmt{
To this end, we first look into a standard state-space model with state $\x_n$ and observation $\y_n$ at each time step $n$. The prior distribution is a Gauss-Markov chain with $p(\x_{n+1}|\x_n) = \N(\x_{n+1}|\A_n\x_n, \Q_n)$ and $p(\x_0) = \N(\x_0|\m_0, \P_0)$. One advantage of the standard state-space model is that, to handle streaming observations $\{ \y_1, \y_2, \ldots \}$, we only need to compute and track the running posterior $p(\x_n | \y_{1:n})$  upon receiving each $\y_n$, where $\y_{1:n} $ denotes the total data up to step $n$.  This is called filtering. Suppose $p(\x_n | \y_{1:n})= \N(\x_n | \m_k, \P_k)$. After all the data has been processed --- suppose it ends after step $N$ --- we can use Rauch–Tung–Striebel (RTS) smoother [] to efficiently compute the full posterior of each state from backward, which does not need to re-access any data:   $p(\x_n|\y_{1:N}) = \N(\x_n | \m_n^s, \P_n^s)$, where 
\begin{align}
	\m^-_{n+1} &= \A_n \m_n, \;\; \P^-_{n+1} = \A_n \P_n \A_n^\top + \Q_n , \notag \\
	\G_n &= \P_n \A_n^\top [\P^-_{n+1}]^{-1}, \notag \\
	\m^s_n &= \m_n + \G_n\left(\m^s_{n+1} - \m^-_{n+1}\right), \notag \\
	\P^s_n &= \P_n + \G_n[\P^s_{n+1} - \P^-_{n+1}]\G_n^\top. \label{eq:rts}
\end{align}
As we can see, the computation only needs the running posterior $p(\x_n|\y_{1:n})=\N(\cdot|\m_n, \P_n)$ and the full posterior of the next state $p(\x_{n+1}|\y_{1:N}) = \N(\cdot | \m_{n+1}, \P_{n+1})$.

Due to the chain structure, the running posterior at step $n$ only relies on  the running posterior at step $n-1$, and has nothing to do with more earlier steps,
\begin{align}
	&p(\x_{n}|\y_{1:n}) \notag \\
	&\propto \int p(\x_{n-1}|\y_{1:n-1}) p(\x_n | \x_{n-1}) p(\y_n | \x_n) \d \x_{n-1}. \label{eq:filter} 
\end{align}
Therefore,  the model update upon receiving an new observation can be very efficient.  We can continuously filter  the data stream. Only when all the data has been processed or we want to extract the state trajectory, we run RTS smoothing to compute the full posterior. This on-demand computation can be done in parallel, as long as we keep track every $p(\x_n | \y_{1:n})$.   When the likelihood $p(\y_n |\x_n)$ is Gaussian, $p(\x_n|\y_{1:n})$ can be computed with a closed Gaussian form, which is called Kalman filtering. 
}


However, one cannot apply  the above framework  outright to our model, since the tensor decomposition likelihood of each observed entry couples the states of multiple factor trajectories (\eg see \eqref{eq:cp-ll} ) --- corresponding to the participated objects in different modes. That means, the factor-state chains of different objects are dynamically intertwined through the received data. The multiplicative form of these states in the likelihood render the running posterior of each trajectory intractable to compute, not to mention running RTS smoother. To address this challenge, we take advantage of the chain structure and use the recent conditional Expectation propagation (CEP) framework~\citep{wang2019conditional} to develop an efficient online filtering algorithm, which approximates  the running posterior of the involved factor states as a product of Gaussian. %each time upon receiving new data. %Due to the factorized structure in the likelihood approximation, the running posterior estimation will also be factorized over each factor state. 
Thereby, we can decouple the involved factor state chains, and conduct standard RTS smoothing for each chain independently. 

%notations, marginalize out ..., and give the formulation, and refer to Zheng's paper --- it is done 
Specifically, denote the sequence of timestamps  when each object $j$ of mode $m$ has showed up in the data stream up to $t_n$, by $s^m_{j, 1} < s^m_{j,2}<\ldots < s^m_{j, c^m_{j,n}}$ where $c^m_{j,n}$ is the object's appearance count up to $t_n$.  \cmt{This is a sub-sequence of $t_1 < \cdots < t_n$. } 
 Denote by $\Ical^m_{n}$ the indexes of all the objects of mode $m$ appearing in $\Bcal_n$, namely, the set of entries received at $t_n$.  Hence, for every object $j \in \Ical^m_n$, we have $s^m_{j, c^m_{j,n}} = t_n$, and $\barz^m_{j, c^m_{j,n}} \overset{\Delta}{=} \z^m_{j}(t_n)$ is the factor state of the object at $t_n$. %Note that $s^m_{j, c^m_{j,n}-1}$ --- the preceding timestamp when the object showed up --- is not necessarily equal to $t_{n-1}$, since it might no appear in $\Bcal_{n-1}$ (see Fig. XX for an illustration). 
Upon receiving each $\Bcal_n$, we intend to approximate the running posterior of all the involved factor states and noise inverse variance $\tau$ with the following decoupled form, 
\begin{align}
p(\tau, \{\barz^m_{j, c^m_{j,n}}| j \in \Ical^m_n\}_{1 \le m \le M}|\Dcal_{t_n}) \approx q(\tau|\Dcal_n)\prod\nolimits_{m=1}^M \prod\nolimits_{j \in \Ical^m_n} q(\barz^m_{j, c^m_{j,n}}|\Dcal_{t_n})  \label{eq:post-n}
\end{align}
where $q(\tau|\Dcal_{t_n}) = \text{Gam}(\tau | a_n, b_n)$, and $q(\barz^m_{j, c^m_{j,n}}|\Dcal_{t_n}) = \N(\barz^m_{j,c^m_{j, n}}|\bmu^m_{j,c^m_{j,n}}, \V^m_{j,c^m_{j,n}})$.
%\begin{align}
	%q(\barz^m_{j, c^m_{j,n}}|\Dcal_{t_n}) = \N(\barz^m_{j,c^m_{j, n}}|\bmu^m_{j,c^m_{j,n}}, \V^m_{j,c^m_{j,n}}).
%\end{align}
To this end, let us consider given the approximation at $t_n$, how to obtain the new approximation  at $t_{n+1}$ (\ie upon receiving $\Bcal_{n+1}$) in the same form of \eqref{eq:post-n}. To simplify the notation, let us define the preceding states of the involved factors by $\Theta_{n} = \{\barz^m_{c^m_{j,n}} | j \in \Ical^m_{n+1}\}_m$, and the current states by $\Theta_{n+1} = \{\barz^m_{c^m_{j,n+1}} | j \in \Ical^m_{n+1}\}_m$. 
First, due to the chain structure of the prior over each $\{\barz^m_{c^m_{j,k}} | k=0, 1, 2, \ldots\}$, we can see that  conditioned on $\{\Theta_n, \tau\}$,   the current states $\Theta_{n+1}$ and the new observations $\Bcal_{n+1}$ are independent  of $\Dcal_{t_n}$. This is because in the graphical model representation, $\{\Theta_n, \tau\}$ have blocked all the paths from the old observations $\Dcal_{t_n}$  to the new state and observations; see Fig. \ref{fig:graphical_model} in Appendix for an illustration. Then, we can drive that 
\begin{align}
	&p(\Theta_{n+1}, \Theta_n, \tau |\Dcal_{t_{n+1}}) \propto p(\Theta_{n+1}, \Theta_{n}, \tau, \Bcal_{n+1}|\Dcal_{t_{n}}) =p(\Theta_n, \tau|\Dcal_{t_n}) p(\Theta_{n+1}, \Bcal_{n+1}|\Theta_{n}, \tau, \Dcal_{t_{n}}) \notag \\
	&=p(\Theta_n, \tau|\Dcal_{t_n}) p(\Theta_{n+1}, \Bcal_{n+1}|\Theta_{n}, \tau) =p(\Theta_n, \tau|\Dcal_{t_n}) p(\Theta_{n+1}|\Theta_{n}) p(\Bcal_{n+1}| \Theta_{n+1}, \tau),
\end{align}
where $p(\Theta_n, \tau|\Dcal_{t_n})$ is the running posterior at $t_n$, $p(\Theta_{n+1}|\Theta_{n}) = \prod_{m=1}^M \prod_{j \in \Ical^m_{n+1}} p(\barz^m_{j,c^m_{j, n+1}}| \barz^m_{j,c^m_{j, n}})$, each $p(\barz^m_{j,c^m_{j, n+1}}| \barz^m_{j,c^m_{j, n}}) $ is a conditional Gaussian distribution  defined in \eqref{eq:state-space}, 
and  $p(\Bcal_{n+1}| \Theta_{n+1}, \tau)=  \prod_{(\bell, y) \in \Bcal_{n+1}} \N\left(y| \1^\top \left(\u^1_{\ell_1}(t_{n+1}) \circ \cdots \circ \u^M_{\ell_M}(t_{n+1})\right),  \tau^{-1}\right)$.

Since $p(\Theta_n, \tau|\Dcal_{t_n})$ takes the form of \eqref{eq:post-n}, we can analytically marginalize out each $\barz^m_{j, c^m_{j,n}} \in \Theta_{n}$, and obtain  
\begin{align}
	&p\left(\Theta_{n+1}, \tau|\Dcal_{t_{n+1}}\right) \propto \text{Gam}(\tau | a_n, b_n)   \prod\nolimits_{m=1}^M \prod\nolimits_{j \in \Ical^m_n}  \N(\barz^m_{j,c^m_{j, n+1}}|\widehat{\bmu}^{m}_{j,c^m_{j,n+1}}, \widehat{\V}^{m}_{j,c^m_{j,n+1}}) \label{eq:running-2}\\
	&  \cdot \prod\nolimits_{(\bell, y) \in \Bcal_{n+1}} \N\left(y| \1^\top \left(\u^1_{\ell_1}(t_{n+1}) \circ \cdots \circ \u^M_{\ell_M}(t_{n+1})\right), \notag \tau^{-1}\right). \notag 
\end{align}
If we view the R.H.S of \eqref{eq:running-2} as a joint distribution with $\Bcal_{n+1}$, then our task amounts to estimating the posterior distribution, \ie the L.H.S of \eqref{eq:running-2}. The product in the CP likelihood (and also Tucker likelihood) renders exact posterior inference infeasible (the normalization constant is intractable). We approximate each likelihood via  
\begin{align}
	&\N\left(y| \1^\top \left(\u^1_{\ell_1}(t_{n+1}) \circ \cdots \circ \u^M_{\ell_M}(t_{n+1})\right)\right) \appropto  \prod\nolimits_{m=1}^M \N\left(\u^m_{\ell_m}(t_{n+1})|\bgamma^m_{\ell_m}, \bSigma^m_{\ell_m}\right)\cdot \text{Gam}(\tau|\alpha_{\bell}, \omega_{\bell}) \label{eq:ll-approx} 
\end{align}
where $\appropto$ means approximately proportional to. To optimize these approximation terms, we use the recent conditional Expectation propagation (CEP) framework~\citep{wang2019conditional} to develop an efficient inference algorithm. It uses conditional moment matching to update each approximation in parallel and conducts fixed point iterations, and hence can converge fast. We leave the details in the Appendix. Once it is done, we substitute the approximation \eqref{eq:ll-approx} into \eqref{eq:running-2}. Then the R.H.S of \eqref{eq:running-2} becomes a product of  Gaussian and Gamma terms over each state and $\tau$. Since both the Gaussian and Gamma distributions are in the exponential family, their product is still in the exponential family. We can immediately obtain a closed-form estimation with the same form as \eqref{eq:post-n}. At the beginning, when estimating $p(\Theta_1, \tau|\Dcal_{t_1})$, since the preceding states $\Theta_0 = \emptyset$,  we have $a_n = \alpha_0$, $b_n = \alpha_1$, $\widehat{\bmu}^{m}_{j,c^m_{j,n+1}} = \0$, and $\widehat{\V}^{m}_{j,c^m_{j,n+1}} = \overline{\P}_\infty$ in \eqref{eq:running-2}, which is the prior of each $\barz^m_{j, c^m_{j,1}}$ and $\tau$ (see \eqref{eq:state-space}). 

In this way, we can continuously filter the incoming batches $\{\Bcal_1, \Bcal_2, \ldots\}$. As a result, for the factor state chain of every object $j$ in every mode $m$, along with each timestamp $s^m_{j, k}$, we can online estimate and track a running posterior approximation $\{q(\barz^m_{j, k} | \Dcal_{t_{s^m_{j,k}}})|k=1, 2, \ldots\}$, which is a Gaussian distribution. Hence, we can run the standard RTS smoother, to compute the full posterior of every factor state, with which we can compute the posterior of the trajectory at any time point $t$~\citep{bishop2006pattern}. Our method is summarized in Algorithm \ref{alg:alg} in Appendix. 

\noindent\textbf{Algorithm Complexity.} The time complexity of our algorithm in processing a batch $\Bcal_n$ is $\Ocal(|\Bcal_n| R^3)$ where $|\cdot |$ denotes the size. The time complexity of RTS smoother for a particular object $j$ in mode $m$ is $\Ocal(R^3 c^m_{j, N})$, where $N$ is the total number of timestamps. The space complexity of our algorithm is $\Ocal(\prod_{m=1}^M \prod_{j=1}^{d_m} c^m_{j, N} (R+R^2))$, which is to track the running posterior of the factor state at each appearing timestamp for every object. Since $c^m_{j, N} \le N$, the complexity of our algorithm is at worst linear in $N$. 
\cmt{
\begin{algorithm}[tb]
	\caption{\ours}
	\label{alg:alg}
	\begin{algorithmic}
		\STATE {\bfseries Input:} kernel hyper-parameters $l,\sigma^2,\nu=p+\frac{1}{2}$
		\STATE Initialize approximation terms in \eqref{eq:llk-approx} for each likelihood.
		\REPEAT
		\STATE  Run KF and RTS smoothing to compute each $q(\barbgam_n)$
		\FOR{$n=1$ {\bfseries to} $N$ in parallel}
		\STATE Simultaneously update $\N(\H\barbgam_{n}|\bbeta_{n}, \S_n)$, $\text{Gam}(\tau|b_n, c_n)$ and $\left\{\N\left(\u_{i_{n_k}}^{k} | \m_{i_{n_k}}^{k,n}, {\V}_{i_{n_k}}^{k,n}\right)\right\}_k$ in \eqref{eq:llk-approx}  with conditional moment matching and multi-variate delta method.
		\ENDFOR
		\UNTIL{Convergence}
		\STATE {\bfseries Return:} $\{q(\Wcal(t_n))\}_{n=1}^N$, $\{q(\u^k_j)\}_{1\le k \le K, 1 \le j  \le d_k}$, $q(\tau)$
	\end{algorithmic}
\end{algorithm}
}
\cmt{
\begin{align}
&p\left(\left\{ \barz^m_{c^m_{j, n+1}}| j \in \Ical^m_{n+1}\right\}_m, \tau|\Dcal_{n+1}\right) \appropto \text{Gam}(\tau | a_n, b_n)\notag \\ 
& \cdot  \prod_{m=1}^M \prod_{j \in \Ical^m_n}  \N(\barz^m_{j,c^m_{j, n+1}}|\widehat{\bmu}^{m}_{j,c^m_{j,n+1}}, \widehat{\V}^{m}_{j,c^m_{j,n+1}}) \notag \\
& \cdot \prod_{(\bell, y) \in \Bcal_{n+1}}\prod_{m=1}^M \N\left(\u^m_{\ell_m}(t_{n+1})|\bgamma^m_{\ell_m}, \bSigma^m_{\ell_m}\right)\cdot \text{Gam}(\tau|\alpha_{n}, \beta_{n})
\end{align}
}
%it is straightforward to obtain a closed-form estimate of  $p\left(\left\{ \barz^m_{c^m_{j, n+1}}| j \in \Ical^m_{n+1}\right\}_m, \tau|\Dcal_{n+1}\right) = $, which has a similar form to  \eqref{eq:post-n}.

\cmt{
We now present our streaming model estimation algorithm.
In general, the observed tensor entries are assumed to be
streamed in a sequence of small batches, {B1, B2, . . .}. Dif-
ferent batches do not have to include the same number of
entries. Upon receiving each batch Bt, we aim to update
the posterior distribution of the factors U, the inverse noise
variance  (for continuous dat
}

